Mood of India During Covid-19 -- An Interactive Web Portal Based on Emotion Analysis of Twitter Data

The severe outbreak of Covid-19 pandemic has affected many countries across the world, and disrupted the day to day activities of many people. During such outbreaks, understanding the emotional state of citizens of a country could be of interest to various organizations to carry out tasks and to take necessary measures. Several studies have been performed on data available on various social media platforms and websites to understand the emotions of people against many events, inclusive of Covid-19, across the world. Twitter and other social media platforms have been bridging the gap between the citizens and government in various countries and are of more prominence in India. Sentiment Analysis of posts on twitter is observed to accurately reveal the sentiments. Analysing real time posts on twitter in India during Covid-19, could help in identifying the mood of the nation. However, most of the existing studies related to Covid-19, on twitter and other social media platforms are performed on data posted during a specific interval. We are not aware of any research that identifies emotional state of India on a daily basis. Hence, we present a web portal that aims to display mood of India during Covid-19, based on real time twitter data. This portal also enables users to select date range, specific date and state in India to display mood of people belonging to the specified region, on the specified date or during the specified date range. Also, the number of Covid-19 cases and mood of people at specific cities and states on specific dates is visualized on the country map. As of May 6 2020, the web portal has about 194370 tweets, and each of these tweets are classified into seven categories that include six basic emotions and a neutral category. A list of Trigger Events are also specified, to allow users to view the mood of India on specific events happening in the country during Covid-19.

==> Mood of India During Covid-19/Tables.tex <==
 \begin{table}[h!]
    \caption{Table 1 - Demographics of volunteers}
    \label{tab:demographics}
    \centering
    \begin{tabular}{|c|c|c|c|}
         \hline
         & Frequency & Percent (\%) & Cummulative (\%)\\
         \hline
         \textbf{Age} & & &\\
         \hline
         18 & 4 & 13.3 & 13.3\\
         19 & 16 & 53.4 & 66.7\\
         20 & 3 & 10 & 76.7\\
         21-23 & 3 & 10 & 86.7\\
         24-25 & 4 & 13.3 & 100 \\
         \hline
         \textbf{Gender}& & &\\
         \hline
         Male & 14 & 46.7 & 46.7\\
         Female & 16 & 53.3 & 100\\
         \hline
         \textbf{Familiarity}& & &\\
         \hline
         Very Familiar & 7 & 23.3 & 23.3\\
         Familiar & 12 & 40 & 63.3\\
         Neutral & 7 & 23.3 & 86.6\\
         Rarely Use e-books & 3 & 10 & 96.6\\
         Never used e-books & 1 & 3.4 & 100\\
         
         \hline
         
         
    \end{tabular}
    
\end{table}

\begin{table}[h!]
    \caption{Table 2 - TAM2+IDT based questionnaire and its results.}
    \label{tab:TAMResults}
    \fontsize{8}{12}\selectfont
    \centering
    \begin{tabular}{|c|c|c|c|}
     \hline
     \textbf{Variable} &\textbf{Question} &\textbf{Mean} &\textbf{SD}
     \\
     \hline
     C & Using DynamiQue is compatible with my reading style & 3.74 & 0.505\\
      &(1=strongly disagree, 5=strongly agree)& &\\
     
    \hline
     C & Using DynamiQue fits well with the way I like to read e-books
    & 3.74 & 0.670\\
      &(1=strongly disagree, 5=strongly agree)& &
    \\
    \hline
     PU & Using DynamiQue would improve my scope of understanding& 3.98 & 0.587
    \\
     & real-time use of concepts in the e-book (1=strongly disagree, 5=strongly agree)& &
     \\
    \hline
     PU & Using DynamiQue would increase my productivity in reading & 3.67 & 0.641\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & Using DynamiQue would enhance my effectiveness in learning & 3.78 & 0.658
     \\
     & and understanding topic of discussion in e-book (1=strongly disagree, 5=strongly agree)& & 
     \\
     \hline
     PU & Using DynamiQue would make it easier for me to learn from e-books & 3.84 & 0.627\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & I think using DynamiQue is very useful for me to learn. & 3.68 & 0.589\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & Questions retrieved by DynamiQue are relevant to the page content & 3.77 & 0.791\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think learning to use DynamiQue is easy & 4.12 & 0.706\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think finding what I want via DynamiQue is easy & 3.78 & 0.749\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think becoming skillful at using DynamiQue is easy & 3.9 & 0.776\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think using DynamiQue is easy & 4.03 & 0.739\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     BI & Assuming I had access to DynamiQue, I intend to use it & 3.74 & 0.620\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     BI & DynamiQue has made my learning interactive & 3.80 & 0.737\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     AU & I would often engage reading e-books via DynamiQue & 3.45 & 0.558\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline

 \end{tabular}
\end{table}
\begin{table}[h!]
\caption{Table 3 - Correlation Analysis Results of TAM2+IDT variables}
    \label{tab:CorrResults}
    \centering
\begin{tabular}{|c c c c c c|}
    \hline
     & C & PU & PEOU & BI & AU \\
     \hline
     C & 1 & & & &\\
     PU & 0.141 & 1 & & &\\
     PEOU & -0.099 & 0.25 & 1 & &\\
     BI & 0.485 & 0.644 & 0.057 & 1 &\\
     AU & 0.299 & 0.576 & 0.421 & 0.563 & 1\\
     \hline
\end{tabular}
\end{table}



==> Tables.tex <==
 \begin{table}[h!]
    \caption{Table 1 - Demographics of volunteers}
    \label{tab:demographics}
    \centering
    \begin{tabular}{|c|c|c|c|}
         \hline
         & Frequency & Percent (\%) & Cummulative (\%)\\
         \hline
         \textbf{Age} & & &\\
         \hline
         18 & 4 & 13.3 & 13.3\\
         19 & 16 & 53.4 & 66.7\\
         20 & 3 & 10 & 76.7\\
         21-23 & 3 & 10 & 86.7\\
         24-25 & 4 & 13.3 & 100 \\
         \hline
         \textbf{Gender}& & &\\
         \hline
         Male & 14 & 46.7 & 46.7\\
         Female & 16 & 53.3 & 100\\
         \hline
         \textbf{Familiarity}& & &\\
         \hline
         Very Familiar & 7 & 23.3 & 23.3\\
         Familiar & 12 & 40 & 63.3\\
         Neutral & 7 & 23.3 & 86.6\\
         Rarely Use e-books & 3 & 10 & 96.6\\
         Never used e-books & 1 & 3.4 & 100\\
         
         \hline
         
         
    \end{tabular}
    
\end{table}

\begin{table}[h!]
    \caption{Table 2 - TAM2+IDT based questionnaire and its results.}
    \label{tab:TAMResults}
    \fontsize{8}{12}\selectfont
    \centering
    \begin{tabular}{|c|c|c|c|}
     \hline
     \textbf{Variable} &\textbf{Question} &\textbf{Mean} &\textbf{SD}
     \\
     \hline
     C & Using DynamiQue is compatible with my reading style & 3.74 & 0.505\\
      &(1=strongly disagree, 5=strongly agree)& &\\
     
    \hline
     C & Using DynamiQue fits well with the way I like to read e-books
    & 3.74 & 0.670\\
      &(1=strongly disagree, 5=strongly agree)& &
    \\
    \hline
     PU & Using DynamiQue would improve my scope of understanding& 3.98 & 0.587
    \\
     & real-time use of concepts in the e-book (1=strongly disagree, 5=strongly agree)& &
     \\
    \hline
     PU & Using DynamiQue would increase my productivity in reading & 3.67 & 0.641\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & Using DynamiQue would enhance my effectiveness in learning & 3.78 & 0.658
     \\
     & and understanding topic of discussion in e-book (1=strongly disagree, 5=strongly agree)& & 
     \\
     \hline
     PU & Using DynamiQue would make it easier for me to learn from e-books & 3.84 & 0.627\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & I think using DynamiQue is very useful for me to learn. & 3.68 & 0.589\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PU & Questions retrieved by DynamiQue are relevant to the page content & 3.77 & 0.791\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think learning to use DynamiQue is easy & 4.12 & 0.706\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think finding what I want via DynamiQue is easy & 3.78 & 0.749\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think becoming skillful at using DynamiQue is easy & 3.9 & 0.776\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     PEOU & I think using DynamiQue is easy & 4.03 & 0.739\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     BI & Assuming I had access to DynamiQue, I intend to use it & 3.74 & 0.620\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     BI & DynamiQue has made my learning interactive & 3.80 & 0.737\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline
     AU & I would often engage reading e-books via DynamiQue & 3.45 & 0.558\\
      &(1=strongly disagree, 5=strongly agree)& &
     \\
     \hline

 \end{tabular}
\end{table}
\begin{table}[h!]
\caption{Table 3 - Correlation Analysis Results of TAM2+IDT variables}
    \label{tab:CorrResults}
    \centering
\begin{tabular}{|c c c c c c|}
    \hline
     & C & PU & PEOU & BI & AU \\
     \hline
     C & 1 & & & &\\
     PU & 0.141 & 1 & & &\\
     PEOU & -0.099 & 0.25 & 1 & &\\
     BI & 0.485 & 0.644 & 0.057 & 1 &\\
     AU & 0.299 & 0.576 & 0.421 & 0.563 & 1\\
     \hline
\end{tabular}
\end{table}


